Prioritizing Speech Test Cases

With the wide adoption of automated speech recognition (ASR) systems, it is increasingly important to test and improve ASR systems. However, collecting and executing speech test cases is usually expensive and time-consuming, motivating us to strategically prioritize speech test cases. A key question is: how to determine the ideal order of collecting and executing speech test cases to uncover more errors as early as possible? Each speech test case consists of a piece of audio and the corresponding reference text. In this work, we propose PROPHET (PRiOritizing sPeecH tEsT), a tool that predicts potential error-uncovering speech test cases only based on their reference texts. Thus, PROPHET analyzes test cases and prioritizes them without running the ASR system, which can analyze speech test cases at a large scale. We evaluate 6 different prioritization methods on 3 ASR systems and 12 datasets. Given the same testing budget, we find that our approach uncovers 12.63% more wrongly recognized words than the state-of-the-art method. We select test cases from the prioritized list to fine-tune ASR systems and analyze how our approach can improve the ASR system performance. Statistical tests show that our proposed method can bring significantly larger performance improvement to ASR systems than the existing baseline methods. Furthermore, we perform correlation analysis and confirm that fine-tuning an ASR system using a dataset, on which the model performs worse, tends to improve the performance more.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/fuzz.tex <==

\subsection{Fuzz Testing Framework for ASR}
\label{subsec:fuzz}
The above method aims at selecting the texts from a large corpus whose corresponding audio is likely to be ASR failure. However, it is constrained to the texts in the corpus only, limiting its ability to uncover more failed test cases. As a result, we propose a fuzz testing framework that can make natural changes to the original texts to generate perturbed texts leading to new ASR failure. We describe the fuzz testing framework as follows.


\begin{algorithm}[!t]
  \caption{Fuzz Testing Algorithm for ASR Systems} 
  \label{algo:fuzz}
  \SetAlgoLined
  \KwInput{$A$: an ASR system under test, $T$: a TTS system, $W$: a word error predictor, $text$: a text whose audio can be correctly transcribed by $A$}
  \KwOutput{$f$: a failed text case for $A$}
  $nouns$ = $POS(text)$ \# extract all nouns in the text using POS\;
  \For(){
    $noun$ {\em in} $nouns$
    }{
        $masked\_text$ = $mask(text, noun)$ \# mask a noun in the text\;
        $substitutes$ = $predict(masked\_text)$\;
        \# get substitutes using the masked language prediction\;
        $ranked\_substitutes$ = $rank(substitutes, W)$\;
        \# rank substitutes using the word error predictor\;
        \For(){
            $sub$ {\em in} $ranked\_substitutes$
        }{
            \# iterate all the substitutes for $ranked\_substitutes$\;
            $text'$ = $replace(masked\_text, sub$)\;
            \# replace the noun in the masked text with the substitute\;
            $audio'$ = $T(text')$\;
            \# synthesize the audio of the new text\;
        \If{$A(audio') \neq text'$}{
          \algorithmicreturn{ $(text', audio')$} \# return the failed test case\;
        }
        }
    } 
  \algorithmicreturn{ $None$}
\end{algorithm}

\subsubsection{Context-aware Replacement for Texts}
\label{subsubsec:natural}

For a correctly recognized pair consisting of a text and a piece of audio, we slightly perturb the text to generate a new text whose audio will be wrongly transcribed by an ASR system (i.e., the transcription does not match the modified text). Such perturbations should ensure the fluency of the revised texts. As described by Li et al.~\cite{bert-attack}, modification for texts needs to be imperceptible to human judges and fluent in grammar. In an extreme case, we can replace most words in a sentence with lengthy and uncommonly used words to generate a text that is very likely to be a failed test case. However, such failed test cases lack practical value for improving the quality of ASR systems. 

The goal of this fuzz framework is to identify the word or combinations of words that may lead to failure, which can provide more insight for the model developers. The model developers can know the reasons for failures and make targeted improvements, e.g., collect more training data that contains erroneous words. To achieve this objective, we need to make the modifications to texts as minimal as possible. As a result, we adopt a very conservative setting: only one word can be modified in each sentence at most. This setting also ensures that the modified texts are very similar to the original texts.

Even only one word is modified, arbitrary substitutions can also make the modified text is a fluent and meaningful English sentence. Figure~\ref{fig:replacement} shows examples of natural and unnatural replacement. The original text is `I have a very cute dog.' An example of unnatural replacement can be to replace `have' with `vasoconstriction,' which produces an disfluent sentence that may uncover ASR errors without practical implications. We limit the replaceable word in a sentence can only be a noun and believe that it should be substituted to natural replacements. To achieve this goal, we use BERT, a context-aware model that is pre-trained on a large corpus of English texts and its masked language prediction function to generate replacements for selected words. Similar methods have been used in adversarial attacks for NLP models~\cite{bert-attack}. These attacks often need to substitute multiple words in a sentence to fool victim models, which may hurt the fluency of generated examples. Our objective is not to simply make an ASR model fail but to uncover words that may lead to failure. So we only modify a single noun in a sentence.

More specifically, we first apply Part-of-Speech (POS) tagging techniques to a given text and obtain labels for each word in the sentence. The labels can be noun, pronoun, verb, adjective, etc. As mentioned earlier, we only care about the nouns in a sentence. For each noun, we replace it with <UNK>, a special token used in BERT to represent an unknown token. This procedure is called `language masking.' Then we feed the masked sentence into BERT and leverage its `masked token prediction' function to predict the potential values of the masked word. BERT returns a ranked list of words, representing the probability of a word fitting into the context. To further ensure the naturalness of replacements, we only select top k words in the list for further substitution. In Figure~\ref{fig:replacement}, we mask the noun `dog' into `<UNK>', and BERT returns 10 natural replacements for the masked token. 


\subsubsection{Fuzz Testing Algorithm}
\label{subsubsec:fuzz}

We also introduce the fuzz testing algorithm that can find more diverse failed test cases. Algorithm 1illustrates the whole process. This fuzz testing framework takes as input an ASR system under test, a TTS system, the failure predictor described in Section~\ref{subsec:error_predictor}, and a text whose corresponding audio can be correctly transcribed by the ASR system. 


As described in Section~\ref{subsubsec:natural}, we first use the POS technique to extract all the nouns in the given text (Line 1). A noun is masked to produce a masked text (Line 3), and then BERT predicts a list of natural substitutes for this masked noun (Line 4). To make the fuzzing process more efficient, we re-rank the substitutes based on their probability of leading to failed test cases (Line 6). We use the word error predictor described in Section 3.2 to compute the probability. However, it is also expensive to query BERT, whose time complexity is $O(N^2)$. So for more efficient computation, instead of feeding the text with a new substitute into BERT, we feed three words into BERT: the substitute along with its surrounding contexts (i.e., the word that is before and after the substitute position, if they exist). The intuition is that an error may not be solely due to the substitute itself; the combination of the substitution and its surrounding contexts can cause the error, e.g., liaison~[x]. But the words that are far from the substitute have much less impact. So we adopt this strategy to reduce time expense and catch errors. 

Besides, the target of this framework is to uncover diverse errors, so we expect the algorithm to avoid selecting the same group of substitutes that are known as errors. Such substitutes may help find more failed test cases but lack the insights to improve model quality further as they reveal limited and similar causes for errors. So we penalize the over-selected substitutes. We maintain a dataset of errors of an ASR system, consisting of error words and their frequency. This dataset can be obtained using prior knowledge (e.g., the results on a test set) or collected during the running of this algorithm. Based on the frequency of substitutes, we add a weight to the score computed by the word error predictor to penalize the over-selected substitutions. After re-ranking, we replace the masked token back to a substitute (Line 10) and use the TTS to synthesize audio (Line 12). If the ASR system cannot correctly transcribe the new synthetic audio (Line 14), we return the text-audio pair as a failed test case (Line 15). Given a large corpus of texts, we need to run this algorithm multiple times.



\subsection{How effective and efficient is the method in generating new failed test cases?}
% \vspace{0.2cm}\noindent\textbf{RQ3. } {\em How effective and efficient is the method in generating new failed test cases via a fuzzing framework?}
\subsubsection{Experiment Design}
We design a fuzzing framework to perturb the texts and aim to generate more failed test cases by improving the error score of a text. We do not find an appropriate baseline to compare as CrossASR mainly serves as a test case selection algorithm rather than a fuzzing framework. The key in our fuzzing framework is to compute a score which is correlated to failed test cases. We can use the error estimator of CrossASR as the baseline method. 

To perturb a text, we can follow BERT-attack to generate natural substitution. Then, we use genetic programming to evaluate the quality of perturbed texts, with error score as the fitness function. Given a set of raw inputs and the same time limit, we evaluate how much more test cases our framework can find. Also, we can adjust the framework so that it can also works for the error estimator in CrossASR. We need to show that our method can generate more test cases. 

We can do some additional analysis as well. First, whether the generated failed test cases can be also used to improve the performance of test cases. Second, the substitutions, are they existing words or new words. If they are existing erroneous words that have been discussed in previous synthetic data, it means we are reusing the errors, suggesting that the generated failed tests are not diverse enough. We actually expect them to be new words, which means that uncover new errors. Besides, we can also analyze whether these new words are in the vocabulary of the ASR model. It will be good if yes. Otherwise, it means that we are uncovering "out-of-vocabulary" words, which is also valuable. 


We can also have some other stop criteria in the fuzzing framework. For now, we generate synthetic data and evaluate them only at the end of the algorithm. Can we do it in the middle? For example, we can have some threshold (middle of the error score in previous experience). 

\subsubsection{Results}
We are expecting some results. First, we need a table to show how many failed test cases our fuzzing framework can additionally generate. In the same table, we can also show that our method can find more than the error estimator used in ASREvolve~\cite{asrevolve}. Then, we fine-tune ASR model on the additionally generated test cases, and see whether our method can achieve better performance on the test data. If all yes, it means that our test case generation method is also good. 

We can have several venn graphs to show the overlap between previously found error words and the error words in the newly generated test cases. If we didn't see a large overlap, or at least there are some new words. We can claim that we are finding new and more diverse errors instead of taking a shortcut (e.g., using known error words to replace).

\begin{tcolorbox}
    \textbf{Answers to RQ3}: Our method can generate more new failed test cases that contain more diverse error than the previous work.
    \end{tcolorbox}
    



\begin{figure}[t]
  {\vspace{-0.5em}}
  \begin{framed}
  \begin{flushleft}
  \small
  \noindent{\textbf{The original text}}
  \newline\noindent{I have a very cute dog.
  }
  \vspace{0.1cm}\newline\noindent{\textbf{An example of unnatural replacement}}
  \newline\noindent{I \underline{\textbf{vasoconstriction}} a very cute dog.
  }
  \vspace{0.1cm}\newline\noindent{\textbf{An example of natural replacement}}
  \newline\noindent{I have a very cute \underline{\textbf{cat}}.
  }
  \vspace{0.1cm}\newline\noindent{\textbf{Top 10 substitutes generated by BERT}}
  \newline\noindent{Input: I have a very cute \underline{\textbf{<UNK>}}.
  }
  \newline\noindent{Top 10 substitutes: \underline{\textbf{cat}}, \underline{\textbf{bird}}, \underline{\textbf{bike}}, ...
  }
  \end{flushleft}
  \end{framed}
  {\vspace{-1em}}
  \caption{An illustrative example of natural and unnatural modification of a text.}
  \label{fig:replacement}
\end{figure}
